Modeling Graphs with Vertex Replacement Grammars

One of the principal goals of graph modeling is to capture the building blocks of network data in order to study various physical and natural phenomena. Recent work at the intersection of formal language theory and graph theory has explored the use of graph grammars for graph modeling. However, existing graph grammar formalisms, like Hyperedge Replacement Grammars, can only operate on small tree-like graphs. The present work relaxes this restriction by revising a different graph grammar formalism called Vertex Replacement Grammars (VRGs). We show that a variant of the VRG called Clustering-based Node Replacement Grammar (CNRG) can be efficiently extracted from many hierarchical clusterings of a graph. We show that CNRGs encode a succinct model of the graph, yet faithfully preserves the structure of the original graph. In experiments on large real-world datasets, we show that graphs generated from the CNRG model exhibit a diverse range of properties that are similar to those found in the original networks.

==> figures/dendro_rules.tex <==
\begin{tikzpicture}[scale=0.75, transform shape]
\node [nt] at (-2,-6.2) {$0$};
\node at (-1.5,-6.15) {$\xrightarrow{\eta_1}$};

\node [inode] (v1) at (-1,-5.7) {};
\node [inode] (v2) at (0,-5.7) {};
\node [inode] (v3) at (0,-6.7) {};
\node [inode] (v4) at (-1,-6.7) {};
\node [inode] (v5) at (-0.5,-6.2) {};
\node [inode] (v6) at (1,-5.7) {};
\node [inode] (v7) at (2,-5.7) {};
\node [inode] (v8) at (2,-6.7) {};
\node [inode] (v9) at (1,-6.7) {};

\draw [iedge] (v1) edge (v2);
\draw [iedge] (v2) edge (v3);
\draw [iedge](v3) -- (v4) -- (v1) -- (v5);
\draw [iedge](v2) -- (v5) -- (v4) -- (v3) -- (v5);
\draw [iedge](v8) -- (v9) -- (v6) -- (v8) -- (v7) -- (v9);
\draw [iedge] (v7) edge (v6);
\draw [iedge] (v2) edge (v6);
\draw [iedge] (v3) edge (v9);

%%%%%

\node [nt] at (4,-8.2) {$2$};
\node at (4.6,-8.2) {$\xrightarrow{\eta_2}$};

\node [inode] (v6) at (6.5,-7.7) {};
\node [inode] (v7) at (5.5,-7.7) {};
\node [inode] (v8) at (5.5,-8.7) {};
\node [inode] (v9) at (6.5,-8.7) {};
\node [textnode] at (5.15,-7.6) {$1$};
\node at (5.15,-8.65) {$1$};

\draw [iedge](v8) -- (v9) -- (v6) -- (v8) -- (v7) -- (v9);
\draw[iedge]  (v7) edge (v6);

%%%%%

\node [nt] at (3.3,-6.2) {$5$};
\node at (4.4,-6.12) {$\xrightarrow{\eta_3, \eta_4, \eta_7, \eta_8}$};
\node [inode] (v1) at (6.5,-6.2) {};
\node [inode] (v4) at (5.5,-6.2) {};
\node [textnode] at (6.5,-5.85) {$2$};
\node [textnode] at (5.5,-5.85) {$3$};

\draw [iedge] (v4) edge (v1);

%%%%%

\node [nt] at (-2,-8.2) {$2$};
\node at (-1.5,-8.2) {$\xrightarrow{\eta_5}$};

\node [inode] (v1) at (-1,-7.7) {};
\node [inode] (v2) at (0,-7.7) {};
\node [inode] (v3) at (0,-8.7) {};
\node [inode] (v4) at (-1,-8.7) {};
\node [inode] (v5) at (-0.5,-8.2) {};
\node [textnode] at (0.35,-8.75) {$1$};
\node[textnode] at (0.35,-7.7) {$1$};

\draw [iedge](v1) -- (v2) -- (v3) -- (v4) -- (v1) -- (v5) -- (v2);
\draw [iedge] (v5) edge (v4);
\draw [iedge] (v3) edge (v5);

%%%%%%

\node [nt] at (1,-8.2) {$5$};
\node at (1.5,-8.2) {$\xrightarrow{\eta_6}$};

\node [inode] (v3) at (3,-8.7) {};
\node [inode] (v4) at (2,-8.7) {};
\node [inode] (v5) at (2.5,-8.2) {};
\node at (1.95,-8.3) {$1$};
\node at (3,-8.3) {$2$};
\node at (2.5,-7.8) {$2$};

\draw [iedge](v4) -- (v3) -- (v5) -- (v4);

\end{tikzpicture}

==> figures/gen.tex <==
\begin{tikzpicture}
\node [textnode] at (-3.5,3.25) {\textsf{Current Graph} $H^\prime$};
\node [textnode] at (4.75,3.25) {\textsf{Current Graph} $H^\prime$};
\node [textnode] at (0,3.25) {\textsf{New Graph} $\hat{H}$};
\node [textnode] at (9,3.25) {\textsf{New Graph} $\hat{H}$};



% step 1
\begin{scope}[shift={(0,0.26)}]
\node [nt, fill=black, text=white] at (-3.8,2) {$\mathbf{0}$};
\node [label=above: $r_1$] at (-2.25,2) {$\Longrightarrow$};

\node [nt] (v1) at (-0.44,2) {$2$};
\node [nt] (v2) at (0.56,2) {$2$};
\draw [iedge] (v1) edge[bend left] (v2);
\draw [iedge] (v1) edge[bend right] (v2);
\end{scope}

% step 2
\begin{scope}[shift={(0,0.26)}]
\node [nt] (v1) at (4.24,2) {$2$};
\node [nt, fill=black, text=white] (v2) at (5.24,2) {$\mathbf{2}$};
\draw [bedge] (v1) edge[bend left] (v2);
\draw [bedge] (v1) edge[bend right] (v2);

\node [label=above: $r_2$] at (6.8,2) {$\Longrightarrow$};
\node [nt] (v1) at (8,2) {$2$};

\node [inode] (f) at (9,2.5) {};
\node [inode] (g) at (10,2.5) {};
\node [inode] (h) at (10,1.5) {};
\node [inode] (i) at (9,1.5) {};
\draw [iedge] (f) -- (g) -- (h) -- (i) -- (f) -- (h);
\draw [iedge] (g) -- (i);
\draw [bedge] (v1) -- (f);
\draw [bedge] (v1) -- (i);
\end{scope}

% step 3
\begin{scope}[shift={(0,0.5)}]
\node [nt, fill=black, text=white] (v1) at (-5,-0.25) {$\mathbf{2}$};
\node [inode] (f) at (-4,0.25) {};
\node [inode] (g) at (-3,0.25) {};
\node [inode] (h) at (-3,-0.75) {};
\node [inode] (i) at (-4,-0.75) {};

\draw [bedge] (v1) -- (f);
\draw [bedge] (v1) -- (i);
\draw [edge] (f) -- (g) -- (h) -- (i) -- (f) -- (h);
\draw [edge] (g) -- (i);

\node [label=above: $r_3$] at (-2.25,-0.25) {$\Longrightarrow$};

\node [inode] (a) at (-1.5,0.25) {};
\node [inode] (b) at (-0.5,0.25) {};
\node [nt] (c) at (-1,-0.5) {$5$};
\node [inode] (f) at (0.5,0.25) {};
\node [inode] (g) at (1.5,0.25) {};
\node [inode] (h) at (1.5,-0.75) {};
\node [inode] (i) at (0.5,-0.75) {};

\draw [iedge] (a) -- (b); 
\draw [iedge] (a) edge[bend left=20] (c);
\draw [iedge] (a) edge[bend right=20] (c);
\draw [iedge] (b) edge[bend right=20] (c);
\draw [iedge] (b) edge[bend left=20] (c);
\draw [bedge] (b) -- (f);
\draw [bedge] (c) -- (i);
\draw [edge] (f) -- (g) -- (h) -- (i) -- (f) -- (h);
\draw [edge] (g) -- (i);
\end{scope}

%% step 4
\begin{scope}[shift={(0,0.5)}]
\node [inode] (a) at (3,0.25) {};
\node [inode] (b) at (4,0.25) {};
\node [nt, fill=black, text=white] (c) at (3.5,-0.5) {$\mathbf{5}$};
\node [inode] (f) at (5,0.25) {};
\node [inode] (g) at (6,0.25) {};
\node [inode] (h) at (6,-0.75) {};
\node [inode] (i) at (5,-0.75) {};

\draw [edge] (a) -- (b);
\draw [bedge] (a) edge[bend left=20] (c);
\draw [bedge] (a) edge[bend right=20] (c);
\draw [bedge] (b) edge[bend right=20] (c);
\draw [bedge] (b) edge[bend left=20] (c);
\draw [edge] (b) edge (f);
\draw [bedge] (c) edge (i);
\draw [edge] (f) -- (g) -- (h) -- (i) -- (f) -- (h);
\draw [edge] (g) -- (i);

\node [label=above: $r_4$] at (6.75,-0.25) {$\Longrightarrow$};

\node [inode] (a) at (7.5,0.25) {};
\node [inode] (b) at (8.5,0.25) {};
\node [inode] (c) at (8.5,-0.75) {};
\node [inode] (d) at (7.5,-0.75) {};
\node [inode] (e) at (8,-0.25) {};

\draw [iedge](c) -- (d) -- (e) -- (c);
\node [inode] (f) at (9.5,0.25) {};
\node [inode] (g) at (10.5,0.25) {};
\node [inode] (h) at (10.5,-0.75) {};
\node [inode] (i) at (9.5,-0.75) {};
\draw [edge] (a) -- (b) -- (f);
\draw [edge] (f) -- (g) -- (h) -- (i) -- (f) -- (h);
\draw [edge] (g) -- (i);
\draw [bedge] (a) -- (e);
\draw [bedge] (b) -- (e);
\draw [bedge] (a) -- (d);
\draw [bedge] (b) -- (c) -- (i);
\end{scope}
%%

\node [hidden] (p1) at (-5,1.38) {};
\node [hidden] (p2) at (10.62,1.38) {};
% \node [hidden] (p3) at (2.25,2.81) {};
% \node [hidden] (p4) at (2.25,0.06) {};

\draw[dotted] (p1) -- (p2); 
% \draw[dotted] (p3) -- (p4); 

\node [textnode] at (-5.6,2.8) {\textbf{\textsf{I}}};
\node [textnode] at (2.6,2.8) {\textbf{\textsf{II}}};
\node [textnode] at (-5.6,1.06) {\textbf{\textsf{III}}};
\node [textnode] at (2.6,1.08) {\textbf{\textsf{IV}}};
\node [textnode] at (-3.75,2.75) {$\mathcal{S}$};
\end{tikzpicture}


==> figures/new_rules.tex <==
\begin{tikzpicture}[scale=0.68, transform shape]

\node [textnode] at (-5.5, 6) {\large{\textsf{\textbf{A}}}};
%% rule 0
\node [nt] at (-5.5,5) {$0$};
\node at (-5,5) {$\xrightarrow{r_1}$};
\node [nt] (v1) at (-4.5,5) {$2$};
\node [nt] (v2) at (-3.5,5) {$2$};
\draw [iedge] (v2) edge[bend left] (v1);
\draw [iedge] (v2) edge[bend right] (v1);

%%

\node [nt] at (-2.5,5) {$2$};
\node at (-1.95,5) {$\xrightarrow{r_2}$};

\node [inode] (f) at (-1.1,5.5) {};
\node [inode] (g) at (-0.1,5.5) {};
\node [inode] (h) at (-0.1,4.5) {};
\node [inode] (i) at (-1.1,4.5) {};
\node [textnode] at (-1.45,5.5) {$1$};
\node [textnode] at (-1.45,4.5) {$1$};
\draw [iedge] (f) -- (g) -- (h) -- (i) -- (f) -- (h);
\draw [iedge] (g) -- (i);

%%%%

\node [nt] at (1,5) {$2$};
\node at (1.5,5) {$\xrightarrow{r_3}$};
\node [inode] (a) at (2,5.5) {};
\node [inode] (b) at (3,5.5) {};
\node [nt] (c) at (2.5,4.55) {$5$};
\node[textnode] at (3.35,5.55) {$1$};
\node[textnode] at (2.5,4.05) {$1$};

\draw [iedge] (a) -- (b);
\draw [iedge] (a) edge[bend left=20] (c);
\draw [iedge] (a) edge[bend right=20] (c);
\draw [iedge] (b) edge[bend right=20] (c);
\draw [iedge] (b) edge[bend left=20] (c);

%%%%%

\node [nt] at (4,5) {$5$};
\node at (4.5,5) {$\xrightarrow{r_4}$};
\node [inode] (v3) at (6,4.5) {};
\node [inode] (v4) at (5,4.5) {};
\node [inode] (v5) at (5.5,5.35) {};
\node at (4.95,4.9) {$1$};
\node at (6,4.9) {$2$};
\node at (5.5,5.75) {$2$};
\draw [iedge] (v3) -- (v4) -- (v5) -- (v3);


%%%%%%%%%

\node [textnode] at (-5.5, 3.45) {\large{\textsf{\textbf{B}}}};

\node [nt] at (-5.5,2.45) {$0$};
\node at (-5,2.45) {$\rightarrow$};
\node [nt] (b) at (-4.5,1.95) {$5$};
\node [nt] (c) at (-3.5,1.95) {$5$};
\node [nt] (a) at (-4,2.95) {$2$};

\draw [iedge] (a) -- (b);
\draw [iedge] (c) -- (a);
\draw [iedge] (b) edge [bend left=35] (c);
\draw [iedge] (b) edge [bend left=10] (c);
\draw [iedge] (b) edge [bend right] (c);
\draw [iedge] (b) edge [bend right=50] (c);
%%%%%%

\node [nt] at (1,2.5) {$5$};
\node at (1.5,2.5) {$\rightarrow$};
\node [inode] (a) at (2,2.5) {};
\node [inode] (b) at (3,2.5) {};
\draw [iedge] (a) edge (b);
\node [textnode] at (2,2.9) {$2$};
\node [textnode] at (3,2.9) {$3$};

%%%%
\node [nt] at (4,2.45) {$5$};
\node at (4.5,2.45) {$\rightarrow$};

\node [inode] (v3) at (6,1.95) {};
\node [inode] (v4) at (5,1.95) {};
\node [inode] (v5) at (5.5,2.8) {};
\node at (4.95,2.4) {$1$};
\node at (6.05,2.4) {$2$};
\node at (5.5,3.2) {$2$};

\draw[iedge] (v3) -- (v4) -- (v5) -- (v3);

%%%%
\node [nt] at (-2.5,2.5) {$2$};
\node at (-2,2.5) {$\rightarrow$};
\node [inode] (f) at (-1.1,3) {};
\node [inode] (g) at (0,3) {};
\node [inode] (h) at (0,2) {};
\node [inode] (i) at (-1.1,2) {};
\node [textnode] at (-1.45,3) {$1$};
\node [textnode] at (-1.45,2) {$1$};

\draw [iedge] (f) -- (g) -- (h) -- (i) -- (f) -- (h);
\draw [iedge] (g) -- (i);

\end{tikzpicture}


==> figures/synthetic_graph.tex <==
\begin{tikzpicture}[scale=0.9, transform shape]
%%
\node [textnode] at (2.6,1.8) {\textbf{\textsf{(A) Example Graph}}};
\node [textnode] at (7.2116,1.8) {\textbf{\textsf{(B) Example CNRG}}};

\begin{scope}[scale=1.25, transform shape, shift={(0,0.8)}]
\node [enode, minimum size=1.5mm] (1) at (1.6,1.8) {};
\node [enode, minimum size=1.5mm] (2) at (1.5,1.4) {};
\node [enode, minimum size=1.5mm] (3) at (1.2,1.7) {};
\node [enode, minimum size=1.5mm] (4) at (2,1.4) {};
\node [enode, minimum size=1.5mm] (5) at (1.8,1) {};
\node [enode, minimum size=1.5mm] (6) at (2.2,1) {};
\node [enode, minimum size=1.5mm] (7) at (2.4,1.8) {};
\node [enode, minimum size=1.5mm] (8) at (2.62,1.38) {};
\node [enode, minimum size=1.5mm] (9) at (2.82,1.78) {};
\node [enode, minimum size=1.5mm] (11) at (1.56,3.2) {};
\node [enode, minimum size=1.5mm] (12) at (1.713,3.659) {};
\node [enode, minimum size=1.5mm] (13) at (1.269,3.564) {};
\node [enode, minimum size=1.5mm] (14) at (1.16,2.8) {};
\node [enode, minimum size=1.5mm] (15) at (0.811,2.488) {};
\node [enode, minimum size=1.5mm] (16) at (0.711,2.931) {};
\node [enode, minimum size=1.5mm] (17) at (0.962,3.285) {};
\node [enode, minimum size=1.5mm] (18) at (0.46,3.4) {};
\node [enode, minimum size=1.5mm] (19) at (0.76,3.7) {};
\node [enode, minimum size=1.5mm] (21) at (3.2,3.2) {};
\node [enode, minimum size=1.5mm] (22) at (3.4,3.6) {};
\node [enode, minimum size=1.5mm] (23) at (3.6,3.2) {};
\node [enode, minimum size=1.5mm] (24) at (3,2.8) {};
\node [enode, minimum size=1.5mm] (25) at (3.4,2.4) {};
\node [enode, minimum size=1.5mm] (26) at (3.6,2.8) {};
\node [enode, minimum size=1.5mm] (27) at (2.6,3.2) {};
\node [enode, minimum size=1.5mm] (28) at (2.964,3.491) {};
\node [enode, minimum size=1.5mm] (29) at (2.544,3.662) {}; 

%\node [fit=(1)(2)(3), dotted, fill=none, draw=red, circle, inner sep=0pt] {};

  \draw [] (1) -- (2);
  \draw [] (1) -- (3);
  \draw [] (1) -- (4);
  \draw [] (1) -- (7);
  \draw [] (1) -- (14);
  \draw [] (2) -- (3);
  \draw [] (4) -- (7);
  \draw [] (4) -- (5);
  \draw [] (4) -- (6);
  \draw [] (7) -- (8);
  \draw [] (7) -- (9);
  \draw [] (7) -- (24);
  \draw [] (14) -- (17);
  \draw [] (14) -- (15);
  \draw [] (14) -- (16);
  \draw [] (5) -- (6);
  \draw [] (8) -- (9);
  \draw [] (24) -- (27);
  \draw [] (24) -- (25);
  \draw [] (24) -- (26);
  \draw [] (11) -- (14);
  \draw [] (11) -- (12);
  \draw [] (11) -- (13);
  \draw [] (11) -- (17);
  \draw [] (11) -- (27);
  \draw [] (12) -- (13);
  \draw [] (17) -- (18);
  \draw [] (17) -- (19);
  \draw [] (27) -- (28);
  \draw [] (27) -- (29);
  \draw [] (15) -- (16);
  \draw [] (18) -- (19);
  \draw [] (21) -- (24);
  \draw [] (21) -- (27);
  \draw [] (21) -- (22);
  \draw [] (21) -- (23);
  \draw [] (22) -- (23);
  \draw [] (25) -- (26);
  \draw [] (28) -- (29);
%\node [dashed, circle, inner sep=0pt, minimum size=21pt, fill=none, draw=red] at (1.43,1.614) {};
%\node [dashed, circle, inner sep=0pt, minimum size=21pt, fill=none, draw=red] at (1.99,1.16) {};
%\node [dashed, circle, inner sep=0pt, minimum size=23pt, fill=none, draw=red] at (2.616,1.616) {};
\end{scope}
%\node [fit=(1) (2) (3) (4) (5) (6) (7) (8) (9), thick, dotted, fill=none, draw=blue, rounded rectangle, inner sep=2.5pt] {};

\begin{scope}[shift={(0.956,1.94)}, scale=0.9, transform shape]
\begin{scope}[shift={(-0.0617,0.1234)}]
\node [nt] at (5.2,3.04) {$0$};
\node at (5.6,3.04) {$\rightarrow$};

\node [nt] (a) at (6.4,2.6503) {$2$};
\node [nt] (b) at (6.8,3.4) {$2$};
\node [nt] (c) at (6,3.4) {$2$};
\draw [iedge] (a) -- (b) -- (c) -- (a);
\end{scope}

\begin{scope}[shift={(0.2234,0.1234)}]
\node [nt] at (7.4,3.04) {$2$};
\node at (7.8,3.04) {$\rightarrow$};

\node [inode] (v3) at (8.6,3.28) {};
\node [inode] (v1) at (8.2,2.68) {};
\node [inode] (v2) at (9,2.68) {};
\draw [iedge] (v1) -- (v2) -- (v3) -- (v1);

\node [textnode] at (8.592,3.6) {$2$};
\node at (9.5,3.08) {$3\times$};
\end{scope} 


\begin{scope}[shift={(-0.0617,-0.2886)}]

\node [nt] at (5.2,1.6022) {$2$};
\node at (5.6,1.58) {$\rightarrow$};

\node [nt] (a) at (6.4,1.932) {$2$};
\node [nt] (b) at (6,1.2) {$3$};
\node [nt] (c) at (6.8,1.2) {$3$};
\draw [iedge] (a) -- (b) -- (c) -- (a);

\node [textnode] at (6,1.644) {$1$};
\node [textnode] at (6.8,1.624) {$1$};
\end{scope}

\begin{scope}[shift={(0.2234,-0.2666)}]
\node [nt] at (7.4,1.58) {$3$};
\node at (7.8,1.5556) {$\rightarrow$};
\node [inode] (v3) at (8.6,1.74) {};
\node [inode, minimum size=1mm] (v1) at (8.2,1.14) {};
\node [inode] (v2) at (9,1.14) {};
\draw [iedge] (v1) -- (v2) -- (v3) -- (v1);
\node [textnode] at (8.6,2.124) {$3$};
\node at (9.5,1.54) {$6\times$};
\end{scope}
\end{scope}

\end{tikzpicture}

